Efficient Uncertainty Modeling for System Design via Mixed Integer Programming

The post-Moore era casts a shadow of uncertainty on many aspects of computer system design. Managing that uncertainty requires new algorithmic tools to make quantitative assessments. While prior uncertainty quantification methods, such as generalized polynomial chaos (gPC), show how to work precisely under the uncertainty inherent to physical devices, these approaches focus solely on variables from a continuous domain. However, as one moves up the system stack to the architecture level many parameters are constrained to a discrete (integer) domain. This paper proposes an efficient and accurate uncertainty modeling technique, named mixed generalized polynomial chaos (M-gPC), for architectural uncertainty analysis. The M-gPC technique extends the generalized polynomial chaos (gPC) theory originally developed in the uncertainty quantification community, such that it can efficiently handle the mixed-type (i.e., both continuous and discrete) uncertainties in computer architecture design. Specifically, we employ some stochastic basis functions to capture the architecture-level impact caused by uncertain parameters in a simulator. We also develop a novel mixed-integer programming method to select a small number of uncertain parameter samples for detailed simulations. With a few highly informative simulation samples, an accurate surrogate model is constructed in place of cycle-level simulators for various architectural uncertainty analysis. In the chip-multiprocessor (CMP) model, we are able to estimate the propagated uncertainties with only 95 samples whereas Monte Carlo requires 5*10^4 samples to achieve the similar accuracy. We also demonstrate the efficiency and effectiveness of our method on a detailed DRAM subsystem.

==> preliminary.tex <==
\section{The M-gPC Surrogate Model}
\label{Preliminaries}
For better understanding, in this section, we take an example of DRAM subsystem (see Figure) to illustrate the the key ideas of building a M-gPC surrogate model.
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Figure/dram_uncert.pdf}
\caption{Uncertainties in DRAM timings (Table~\ref{Tb:DRAM_para_set}). Note that the timings are not proportional to real values.}\label{fig:dram}
\end{figure}
%\cwl{Hi weilong, plz help check the terms in this section. Also, can we put a figure which can represent the uncertainty in DRAM here?}
%\zz{You cannot describe this part in this way. Your focus should be how to modify the traditional gPC to fit the architecture design problems.}

\subsection{M-gPC Expansion}
\label{sec:gpc_expansion}


% , $Y = \left[ {{y_1},{y_2}, \ldots ,{y_n}} \right]^T \in {\mathbb{R}^n}$ is a vector of model outputs of interest, like the bandwidth or power of the system. 


% One direct approach to approximate $y(\vecpar)$ is by the Monte Carlo method. However, Monte Carlo approach requires a lot of samples to get a high accuracy. Instead,  
%Suppose the stochastic output function $y(\vecpar)$ is smooth and has a bounded variance, we then can approximate it as follows: 
Given a stochastic output function $y(\vecpar)$, we can approximate it as follows:
\begin{equation}\label{eq:gPC_expansion}
  y(\vecpar) \approx  \sum\limits_{\left| {\basisInd} \right| = 0}^p c_{\basisInd}\multiGPC_{\basisInd}(\vecpar) = \sum\limits_{k=1}^{N_p}c_k\multiGPC_k(\vecpar),
\end{equation}
% When the inputs are of stochastic uncertainties, the output analysis becomes a challenge. 
% In a M-gPC approach, a particular model output $y$ can be approximated by a surrogate model ${\tilde Y}$ which is constructed by an expansion of orthogonal basis functions:
% \begin{equation}\label{eq:gPC_expansion}
% y \approx \tilde y = \sum\limits_{\left| {\vec \alpha } \right| = 0}^p {{c_{\vec \alpha }}{\Psi _{\vec \alpha }}\left( {{\rm{ \vecpar}}} \right)}  = \sum\limits_{k = 1}^{{N_p}} {{c_k}{\Psi _k}\left( {{\rm{ \vecpar}}} \right)},
% \end{equation}
where $\multiGPC_{\basisInd}(\vecpar)$ are the multivariate orthogonal basis functions, $c_\basisInd$ are the M-gPC coefficients to be computed, $p$ is the order of M-gPC expansion, and $\basisInd=[\alpha_1,\ldots,\alpha_d]^T$ is an index set for polynomial degrees, leading to $N_p=\binom{d+p}{p}$ expansion terms. 

% One immediate advantage of model \reff{eq:gPC_expansion} is that the mean value and standard derivation of $y(\vecpar)$ has a closed form

% The index ${\vec \alpha}$ has an one-to-one correspondence to any integer $k \in \left[ {1,{N_p}} \right]$, leading to a total number of $N_p=\binom{p+d}{d}$ 
% ${N_p} = \left( {\begin{array}{*{20}{c}}
% {p + d}\\
% d
% \end{array}} \right)$

% basis functions under a total degree scheme~\cite{xiu2010numerical}. \ccf{what is a total degree scheme? }
% \hzc{Actually, M-gPC expansion has exactly the same form with traditional gPC expansion, but the difference .} 

% Once the surrogate model is constructed, we can 


\subsection{Constructing the Basis Functions}\label{sec:basis}
Given the marginal probability density function $\rho_i\left( {{\parm_i}} \right)$ for each variable $\parm_i$, a set of univariate orthornormal polynomials ${\left\{ {\phi _m^{\left( i \right)},m \in \mathbb{N}} \right\}}$ can be constructed 
% Given any input distribution, \hzc{no matter discrete or continuous}, the univariate basis function can be constructed
by a well-known three-term recurrence relation~\cite{gautschi1982generating} (see appendix \ref{sec:TTR}), which satisfy: 
% ${\left\{ {\phi _m^{\left( i \right)},m \in \mathbb{N}} \right\}}$ is a set of orthornormal polynomials:
\begin{equation}
    \mathbb{E}[\phi_{m}^{(i)}\phi_{n}^{(i)}]=\delta_{m,n}, \ \forall\, i=1,\ldots,d.
\end{equation}
% \begin{equation}
% \left\langle {\phi _m^{\left( i \right)},\phi _n^{\left( i \right)}} \right\rangle  = \int\limits_\mathbb{R} {\phi _m^{\left( i \right)}\left( {{\parm_i}} \right) \cdot \phi _n^{\left( i \right)}\left( {{\parm_i}} \right)}  \cdot \rho \left( {{\parm_i}} \right)d{\parm_i} = {\delta _{m,n}},
% \end{equation}
Here, index $m$ and $n$ denote the polynomial degrees, and ${\delta_{m,n}}$ is a Delta function. 
Especially, the basis functions for discrete variable are also defined in a discrete or integer domain. Hence, the corresponding ${\parm_i}$ should also be discrete or an integer. 
%\hzc{When all the inputs are assumed mutually independent, do we need to claim it here?} a multivariate basis function can be constructed based on the products:
A multivariate basis function can then be constructed based on the product of univariate ones:
\begin{equation}
{\Psi _{\basisInd}}\left( \vecpar \right) = \prod\limits_{i = 1}^d {\phi _{{\alpha _i}}^{\left( i \right)}} \left( {{\parm_i}} \right).
\end{equation}

%\ccf{For the discrete parameters in the computer architecture problems, the basis functions are defined on the discrete domain. In such cases, the key difference from their continuous counterpart is?}




\subsection{Stochastic Collocation}
\label{sec:stoc_col}
Stochastic collocation is an efficient choice to compute M-gPC coefficients. %, which is a sampling-based method. 
%Xiu summaries three methods in SC: interpolation, regression and pseudo projection. 
%Among them, the pseudo projection is remarkably robust and accurate, which computes the coefficients ${c_k}$ as:
The key idea is to compute the   coefficients by a robust and accurate projection approach~\cite{Xiu2017}:
\begin{equation}\label{eq:pseudo_proj}
 {c_k} = \mathbb{E}\left[ {y\left( {\vecpar} \right){\Psi_k}\left( {\vecpar} \right)} \right]  \approx \sum\limits_{i = 1}^M {y\left( {{{\vecpar}_i}} \right)} {\Psi _k}\left( {{{\vecpar}_i}} \right){w_i},
%\int\limits_{{\mathbb{R}^d}} {y\left( {\vecpar} \right){\Psi _k}\left( {\vecpar} \right)\rho \left( {\vecpar} \right)d} \vecpar,
\end{equation}
% where $\rho \left( {\vecpar} \right)$ is a joint probability density function of all components in ${\vecpar}$. 
% The crucial point is to find a high-dimensional quadrature rule to approximate the integral (Eq. (\ref{eq:pseudo_proj})):
% \begin{equation}\label{eq:sum_pseudo_proj}
% {c_k} \approx \sum\limits_{i = 1}^M {y\left( {{{\vecpar}_i}} \right)} {\Psi _k}\left( {{{\vecpar}_i}} \right){w_i},
% \end{equation}
where $\left\{ {{{\vecpar}_i}} \right\}_{i = 1}^M$ are the quadrature points and $\left\{ {{w_i}} \right\}_{i = 1}^M$ are the corresponding quadrature weights.

In other words, we only requires $M$ simulation points to build our surrogate model M-gPC. 
In computer architecture design, each circle accurate simulation (points ${\vecpar_i}$) may require several hours or days to run a simulator. 
Henceforth, a good quadrature rule to select small number of sample points with high accuracy is required. 
However, existing quadratures cannot generate mixed-integer points to fit both continuous and discrete uncertain inputs. 


% In our proposed framework, $M$ is optimized through our proposed algorithm. The preliminary numerical experiments show that our proposed approach only needs dozens or hundreds of sample points  to achieve a similar accuracy with Monte Carlo methods of  $10^5$  points.  
% \ccf{The difference between discrete points and the continuous points}.


% Based on the obtained coefficients, the mean value and standard deviation of the output $y$ can be easily captured as:
% \begin{equation}\label{moments}
% \begin{array}{l}
% \mathbb{E}\left[y \right] \approx {c_1},\;
% \sigma \left( y \right) \approx \sqrt {\sum\limits_{k = 2}^{{N_p}} {{{\left| {{c_k}} \right|}^2}} } 
% \end{array}.
% \end{equation}

==> related_works.tex <==
\section{Related works}
\label{related works}
\subsection{Uncertainty analysis in computer architecture}
There exists extensive existing work on quantifying uncertainty in architecture and system design for different components. Among this line of work, Borkar et. al.~\cite{Borkar:2003:PVI:775832.775920} identify and quantify the PVT variations and their impact on clock frequency of a microprocessor. Bhardwaj and Vrudhula ~\cite{Bhardwaj:2005:LMN:1065579.1065719} study and quantify the impact of process variation on leakage at the circuit level. Zhang et. al.~\cite{Zhang:2009:PVC:1629911.1630092} quantify the uncertainty in leakage power consumption in a chip-multiprocessor under process variation. Wong et. al.~\cite{Wong:2005:FDA:1129601.1129608} use analytic models to quantify the uncertainty in delay and power of FPGA devices under process variation. Das et. al.~\cite{das2007mitigating} quantify latency uncertainty in different micro-architectural units and propose cache mechanisms to improve batch performance under process variations. Yan et. al.~\cite{7271059Yan} propose CoreRank to characterize and manage dynamic performance uncertainty introduced by silicon aging and degradation. Ozdemir et. al.~\cite{4041832} propose yield-aware architectural mechanisms for data cache to combat lower yield rate due to process variation. Liang et. al.~\cite{4408242} designs a new 3T1D cache architecture to mitigate and mask process variation in caches. Regarding a all-around view of uncertainty propagation in system designs, Cui and Sherwood~\cite{Cui:2017:EUA:3123939.3124541} uses analytic models and Monte Carlo simulations to study the scaling trends and trade-offs of uncertainties in a CMP using a very high-level analytic model. In our work, we for the first time look at the uncertainty impact in a DRAM subsystem with accurate detailed simulation data.

\subsection{Quadrature and uncertainty quantification techniques}
%The contents in this subsection will be updated, mainly about discrete gPC and quadrature, and some limitations and challenges.

%Generally speaking, there are two kinds of quadrature: deterministic rule and optimization-based methods. 
The quadrature rules for one dimensional case, like Gauss quadrature rule which can achieve a degree of exactness\footnote{A degree of exactness refers to the highest degree polynomial that can be integrated exactly for a given number of points $m$~\cite{gautschi1981survey}.} of (2m-1) for $m$ points, have been well studied. 
% univariate quadrature rule
But it meets a challenge of scaling up to high-dimensional cases. 
For example, to compute gPC coefficients, the tensor product rule of Gauss quadrature will lead to ${(p+1)^d}$~\cite{xiu2009fast} points in total, which suffers the curse of dimensionality.  

Optimization-based approach offers a good strategy to find multivariate quadrature. 
Ryu and Boyd~\cite{ryu2015extensions} proposed a linear Programming to extend Gaussian quadrature via moment matching method. 
An efficient algorithm to generate multivariate quadrature rules with positive weights was designed by Jakeman and Narayan~\cite{jakeman2018generation}. 
Kseshavarzzadeh \etal~\cite{keshavarzzadeh2018numerical} proposed a computing framework for multivariate positive rule on general geometries.
Cui and Zhang~\cite{cui2018stochastic} designed an optimization-based quadrature for non-Gaussian correlated inputs.

Limitation: order scaling, dimension scaling, function smoothness


